SAM3D: Segment Anything Model in Volumetric Medical Images

Image segmentation remains a pivotal component in medical image analysis, aiding in the extraction of critical information for precise diagnostic practices. With the advent of deep learning, automated image segmentation methods have risen to prominence, showcasing exceptional proficiency in processing medical imagery. Motivated by the Segment Anything Model (SAM)-a foundational model renowned for its remarkable precision and robust generalization capabilities in segmenting 2D natural images-we introduce SAM3D, an innovative adaptation tailored for 3D volumetric medical image analysis. Unlike current SAM-based methods that segment volumetric data by converting the volume into separate 2D slices for individual analysis, our SAM3D model processes the entire 3D volume image in a unified approach. Extensive experiments are conducted on multiple medical image datasets to demonstrate that our network attains competitive results compared with other state-of-the-art methods in 3D medical segmentation tasks while being significantly efficient in terms of parameters. Code and checkpoints are available at https://github.com/UARK-AICV/SAM3D.

==> tex/method.tex <==
\section{Method}
\label{sec:Method}

In this section, we will introduce our model, termed SAM3D, as well as explain the reasoning behind this simple design. In short, our goal is to design a simple adaptation of SAM such that the model should take advantage of SAM without having to re-train too many parameters or construct too complicated and task-specific modules.

\subsection{Overall Architecture}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{images/overall.pdf}
\caption{Overall architecture of the proposed SAM3D, including two modules, i.e., \emph{2D image encoder}, which is derived from Segment Anything Model without any modification, and \emph{3D lightweight decoder}, which utilizes 3D convolutional blocks to incorporate depth-wise information to infer the prediction. In this context, $H, W$, and $D$ respectively represent the input height, width, and depth.} 
\label{fig:SAM3D}
\end{center}
\end{figure*}

% First, let us introduce the general architecture of our method, which is shown in Figure \ref{fig:SAM3D}.

SAM owns a powerful image encoder that can extract meaningful feature representations for natural images. Unfortunately, when it comes to 3D medical images, we observe that the difference between the two domains makes it inappropriate to hope that the original SAM image encoder can extract the true semantic information of the medical images. However, we hypothesize that the feature representation from the SAM image encoder is not completely useless. It contains both high-level features, which are meaningless in the medical image domain, and low-level features including edges, boundaries, blobs, regions, etc. which are still valuable in every image domain. As a consequence, we find it tempting to keep the SAM image encoder unchanged and just use another decoder so that we are able to minimize the number of parameters that need to be trained.

Unlike SAMed and MedSAM \cite{samed, medsam}, instead of finetuning all 3 components of SAM, our method leverages the original SAM's image encoder as the feature extractor in a slice-by-slice fashion and a lightweight 3D image decoder, as depicted by in Figure \ref{fig:SAM3D}. Specifically, the input has resolution $H\times W\times D$, split into $D$ 2D slices which are triplicated into $H\times W\times 3$ with 3 identical channels so that it can be put through SAM's image encoder. The feature maps extracted by the image encoder are stacked into a 3D feature map $H\times W\times D\times C$ where $C$ is the number of channels.
As SAM's mask encoder is designed for 2D image segmentation, we decided to replace it with a 3D lightweight decoder. The 3D feature map is processed by this lightweight decoder to produce the final prediction. In this way, the depth-wise information is efficiently incorporated so that the decoder can learn more and exploit better the anatomical structures.
We also observe different medical image modalities have their own distinct characteristics. As a result, using the prompt encoder may degrade the performance since it hinders the extracted feature from obtaining distinctive information that varies by modality. For that reason, we remove the prompt encoder and use a decoder with a simple classifier.


\subsection{Encoder}
As mentioned before, the feature extracted by SAM's image encoder is supposed to have robust and valuable low-level information regardless of the image domain. Thus, it is plausible to tackle the notorious weak boundary in the medical image domain by using features extracted by SAM's image encoder.
Furthermore, although the difference between 3D medical images and 2D natural images is so large that it seems necessary to finetune the image encoder, any modification to the weights of the encoder might degrade the quality of the extracted low-level feature. Therefore, we freeze the image encoder and train a new lightweight decoder. In Section \ref{sec:Experiment}, we will show that this approach can utilize the information about the texture, intensity, contrast between regions, etc. to effectively construct semantic information specific to 3D medical images and thus yield precise segmentation results.


Formally, let $I\in\mathbb{R}^{H\times W\times D}$ be the input, and $Enc$ denote the image encoder. First, $I$ is split along the depth dimension into $D$ slices. Each $i$-th slice is triplicated to have 3 identical channels, denoted by $I_i\in 3\times H\times W$. $Enc$ takes $I_i$ as input and outputs corresponding slice embedding.

\begin{equation}
    f_i=Enc(I_i), \text{where }f_i\in\mathbb{R}^{\frac{H}{16}\times\frac{W}{16}\times 256}
\end{equation}
We stack these slice embeddings and transpose the result to obtain the final 3D image embedding.
\begin{equation}
    f\in\mathbb{R}^{\frac{H}{16}\times\frac{W}{16}\times D\times 256}
\end{equation}

\subsection{Decoder}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{images/SAM3D-decoder.drawio.pdf}
\caption{Architecture of the 3D lightweight decoder.} 
\label{fig:decoder}
\end{center}
\end{figure*}
% Ở đây mục tiêu thiết kế là chọn ra một lightweight decoder. để giảm số lượng param và deal được với 3D
Because our decoder must have the ability to deal with 3D patches, we cannot take advantage of SAM's mask decoder which is tailored to 2D natural images but choose another decoder and train it from scratch. Vision Transformer \cite{vit2020} and its variants are excluded due to its quadratic computational complexity in terms of the number of patches. It is notable that the number of patches is now $D$ times greater than itself in 2D settings, where $D$ is up to hundreds. Therefore, we decided to use a simple decoder having 4 3D convolutional blocks with skip connections \cite{resnet} and a segmentation head, as illustrated in detail by Figure \ref{fig:decoder}.

\subsection{Objective Function}

Following nnFormer \cite{nnformer}, we utilize both dice loss and cross-entropy loss as loss functions to train our network. It is defined as follows:

\begin{equation}
\begin{split}
    \mathcal{L}(X, Y) = - \sum_{i=1}^{I} \left( 
    \frac{2 \times \sum_{j=1}^{J} X_{j, i} Y_{j, i}} {\sum_{j=1}^{J} X_{j, i} ^ 2 + \sum_{j=1}^{J} Y_{j, i} ^ 2} \right. \\
    \left. + \sum_{j=1}^{J} X_{j, i} log Y_{j, i} \right)
\end{split}
\end{equation}

where, $I$ is the number of classes, $J$ denotes the number of voxels, $X_{j,i}$ and $Y_{j, i}$ denote the ground truths and predictions at voxel $j$ for class $i$, respectively.

We also adopt the deep supervision technique for multiple decoding stages. Specifically, the output features of each decoding stage are passed through the segmentation block, including one 3 x 3 x 3 and one 1 x 1 x 1 convolution layer, to generate the prediction of one typical stage. To calculate the loss value at one typical stage, we down-sample the ground truth equal to the prediction resolution. Therefore, the final loss can be defined as follows:

\begin{equation}
    \mathcal{L}_{total} = \sum_{i=1}^{n} \alpha_{i} \times \mathcal{L}_{i}
    % \mathcal{L}_{all} = \alpha_{1}\mathcal{L}_{1} + \alpha_{2}\mathcal{L}_{2} + \alpha_{3}\mathcal{L}_{3}
\end{equation}

where n, which we set equal to 3, is the number of decoder layers. $\alpha_{i}$ denotes the hyper-parameter to control the contribution of different resolutions to the final loss function. In practice, $\alpha_{2} = \frac{\alpha_{1}}{2}$ and $\alpha_{3} = \frac{\alpha_{1}}{4}$ and all $\alpha$ hyper-parameters are normalized to 1. 
